On-line Adaptative Curriculum Learning for GANs

Generative Adversarial Networks (GANs) can successfully approximate a probability distribution and produce realistic samples. However, open questions such as sufficient convergence conditions and mode collapse still persist. In this paper, we build on existing work in the area by proposing a novel framework for training the generator against an ensemble of discriminator networks, which can be seen as a one-student/multiple-teachers setting. We formalize this problem within the full-information adversarial bandit framework, where we evaluate the capability of an algorithm to select mixtures of discriminators for providing the generator with feedback during learning. To this end, we propose a reward function which reflects the progress made by the generator and dynamically update the mixture weights allocated to each discriminator. We also draw connections between our algorithm and stochastic optimization methods and then show that existing approaches using multiple discriminators in literature can be recovered from our framework. We argue that less expressive discriminators are smoother and have a general coarse grained view of the modes map, which enforces the generator to cover a wide portion of the data distribution support. On the other hand, highly expressive discriminators ensure samples quality. Finally, experimental results show that our approach improves samples quality and diversity over existing baselines by effectively learning a curriculum. These results also support the claim that weaker discriminators have higher entropy improving modes coverage. Keywords: multiple discriminators, curriculum learning, multiple resolutions discriminators, multi-armed bandits, generative adversarial networks, smooth discriminators, multi-discriminator gan training, multiple experts.

==> background.tex <==
% \subsection{GANs}

% A generator $G: \cZ \rightarrow \cX$ receives a noise sample $z \sim p(z)$ where $p(z)$ is a tractable probability density and maps it to the data space $\cX$, resulting in what is referred to as a \emph{generated sample}. A discriminator $D: \cX \rightarrow [0,1]$ maps a data sample to the probability that it was obtained from the true distribution $f_\cX$, rather than being generated by $G$. The tuple $(G,D)$ is fitted through alternating or simultaneous gradient descent updates to minimize the following loss function:
% \begin{align}
%     \min_G\max_D &V(D,G) =
%     \nonumber\\
%     \min_G\max_D & \underset{{x \sim f_\cX(x)}}{\Esp}[\log(D(x))] +
%     \underset{{x \sim G(z)}}{\Esp}[\log(1-D(x))],
%     \label{eq:gan_loss}
% \end{align}
% % where $f_\cX$ is the true data distribution.


% \subsection{Multi-Armed Bandit}

% A Multi-Armed Bandit (MAB) \cite{Robbins1952} problem is described by a finite set of actions $\cA$. During each episode $t\in\Nat_{>0}$ of an episodic MAB game, a player selects an action $a_t\in\cA$ and observes an outcome $y_t\in\cY$, where $\cY \subset\Real$. The goal of this agent consists in maximizing the sum of the outcomes $\sum_{t=1}^T y_t$ over time.


% \paragraph{Stochastic bandits.}

% In the stochastic setting, each action $a\in\cA$ is associated with an expected outcome $\mu_a$, and the outcome $y_t$ has expectation $\mu_{a_t}$. The expected sum of outcomes can therefore be maximized by selecting the action $a^\star = \argmax_{a\in\cA} \mu_a$ on each episode $t$.


% \paragraph{Non-stationary bandits.}

% In the non-stationary stochastic bandits~\cite{besbes2014} case, each action $a\in\cA$ is associated with mean $\mu_{a,t}$ on time $t$. Therefore, the expected sum of outcomes is now maximized by selecting the action $a_t = \argmax_{a\in\cA} \mu_{a,t}$ at time $t$.

